Summing Up Smart Transitions

Some of the most significant high-level properties of currencies are the sums of certain account balances. Properties of such sums can ensure the integrity of currencies and transactions. For example, the sum of balances should not be changed by a transfer operation. Currencies manipulated by code present a verification challenge to mathematically prove their integrity by reasoning about computer programs that operate over them, e.g., in Solidity. The ability to reason about sums is essential: even the simplest ERC-20 token standard of the Ethereum community provides a way to access the total supply of balances. Unfortunately, reasoning about code written against this interface is non-trivial: the number of addresses is unbounded, and establishing global invariants like the preservation of the sum of the balances by operations like transfer requires higher-order reasoning. In particular, automated reasoners do not provide ways to specify summations of arbitrary length. In this paper, we present a generalization of first-order logic which can express the unbounded sum of balances. We prove the decidablity of one of our extensions and the undecidability of a slightly richer one. We introduce first-order encodings to automate reasoning over software transitions with summations. We demonstrate the applicability of our results by using SMT solvers and first-order provers for validating the correctness of common transitions in smart contracts.

==> cleveref/README <==
cleveref, a LaTeX package for intelligent cross-referencing
Copyright (C) 2007--2018  Toby Cubitt

Files:
cleveref.ins  Batch file, run through LaTeX
cleveref.dtx  Docstrip archive, run through LaTeX
cleveref.sty  LaTeX package, generated by cleveref.ins from cleveref.dtx
cleveref.dvi  Package documentation, generated from cleveref.dtx
cleveref.pdf  Package documentation; can also be generated from cleveref.dtx
README        This file

E-mail:   toby-cleveref@dr-qubit.org
Address:  Department of Computer Science, UCL, United Kingdom

This material is subject to the LaTeX Project Public License. See
http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the
details of that license.


Description:
------------
The cleveref package enhances LaTeX's cross-referencing features, allowing the
format of cross-references to be determined automatically according to the
"type" of cross-reference (equation, section, etc.) and the context in which
the cross-reference is used. The formatting for each cross-reference type can
be fully customised in the preamble of your document. In addition, cleveref
can type-set cross-references to lists of multiple labels, automatically
formatting them according to their types, sorting them, and compressing
sequences of numerically consecutive labels. Again, the multiple-reference
formatting is fully customisable. Though a number of other packages provide
similar features, all have certain deficiencies which cleveref attempts to
overcome.

Using cleveref is easy. Basically, wherever you would previously have used
\ref, you can use \cref instead. (Except at the beginning of a sentence, where
you should use \Cref.)  You no longer need to put the name of the thing you're
referencing in front of the \cref command, because cleveref will sort that out
for you: i.e. use "\cref{eq1}" instead of "eq.~(\ref{eq1})". If you want to
refer to a range of labels, use the \crefrange command: "\crefrange{eq1}{eq5}"
produces "eqs.~(1) to~(5)". Finally, if you want to refer to multiple things
at once, you can now combine them all into one cross-reference and leave
cleveref to sort it out: e.g. "\cref{eq2,eq1,eq3,eq5,thm2,def1}" produces:
"eqs.~(1) to~(3) and~(5), theorem~5, and definition~1".

Cleveref has various other useful features. For details, see the package
documentation.


==> includes/floats/2cm-in-sl-fig.tex <==

\newcommand{\addrnodes}[6]{%
\node[state,#6] (#1) [#2] {#3};
\node (#1-val) [above right = 0.5cm and 0cm of #1] {#4};
\node (#1-label) [below = 1cm of #1] {#5};
\node (#1-card) [below right = 2mm and 12mm of #1] {$1$};
\path [->]
	(#1) 
		edge [bend left] node [below right = -1.5mm and 0.5mm] {$g(\cdot)$} (#1-val.west)
		edge [] node [right] {$l(\cdot)$} (#1-label)
		edge [bend left] node [below left = 0mm and -2mm] {$c(\cdot)$} (#1-card)
;
}

\newcommand{\neworrenewcommand}[1]{\providecommand{#1}{}\renewcommand{#1}}

\newcommand{\foo}[9]{
	\neworrenewcommand{\ffoo}[1]{
		#1 #2 #3 #4 #5 #6 #7 #8 #9 ##1
	}
	\ffoo
}

\newcommand{\stepnodes}[9]{
	\neworrenewcommand{\innerstepnodes}[4]{
	
	\node (focus-#1) [#2, minimum width = 10cm] {};
		
	\addrnodes{sep-#1}{below left = -8mm and 2mm of focus-#1}{##1}{0}{#4}{accepting}
	\addrnodes{c1-#1}{right = 2.5cm of sep-#1}{##2}{$c_1$ at \##3}{#5}{}
	\addrnodes{c2-#1}{right = 2.5cm of c1-#1}{##3}{$c_2$ at \##3}{#6}{}
	\addrnodes{pc-#1}{right = 2.5cm of c2-#1}{##4}{#9}{#7}{}
	
	\node[draw=black, 
	fit=
		(focus-#1),
	inner sep=2cm
	](step-#1) {};
	
	\node[above right, inner sep=2pt] at (step-#1.north west) {#8};
	}

	\innerstepnodes
}

\begin{figure}
	\centering
	\begin{tikzpicture}[
		> = stealth,
		semithick,
		node distance = 2cm
	]
		
		\stepnodes{0}{}
			{0}{0}{1}{2}{3}
			{Initial State (Time-step \#0)}
			{$\textsc{pc}=1$}
			{}{}{}{$a_0$}
		
		\stepnodes{1}
			{below = 6cm of focus-0}
			{$i$}{$4i$}{$4i+1$}{$4i+2$}{$4i+3$}
			{Time-step \#$i$}
			{\textsc{pc} at \#$i$}
			{$x_1$}{$x_2$}{$x_3$}{$x_4$}
		
		\stepnodes{2}
			{below = 5cm of focus-1}
			{$(i+1)$}{$4i+4$}{$4i+5$}{$4i+6$}{$4i+7$}
			{Time-step \#$(i+1)$}
			{\textsc{pc}}
			{$x_5$}{$x_6$}{$x_7$}{$x_8$}
			
		\stepnodes{3}
			{below = 6cm of focus-2}
			{$n$}{$s_c - 4$}{$s_c - 3$}{$s_c - 2$}{$s_c - 1$}
			{Final State (Time-step \#$n = \frac{s_c}{4} - 1$)}
			{$\textsc{pc}=H$}
			{}{}{}{$a_1$}
		
		
		\path [->>]
		(step-0) edge[densely dashed] (step-1)
		(step-1) edge (step-2)
		(step-2) edge[densely dashed] (step-3)
		;
	\end{tikzpicture}
	\caption{Transition System of a 2-Counter Machine in SL}
	{\small Each $\bigcirc$ represents an \Addr{}, doubled vertices are separators.}
	\label{fig:2cm-in-sl}	
\end{figure}

==> includes/oldabstract.tex <==
%Context
Some of the most significant high-level properties of currencies are
the sums of certain account balances.
Properties of such sums can ensure the integrity of currencies and transactions.
For example, the sum of balances should not be changed by a transfer operation.
Both crypto-currencies and currencies manipulated by code present a verification challenge to
mathematically prove the integrity of currencies by reasoning about computer programs that manipulate them, e.g., in Solidity.
The ability to reason about sums is essential:
even the simplest token standard, ERC-20 of the Ethereum community,
provides a way to access the total supply.



%Gap
Unfortunately, reasoning about code written against this interface is non-trivial:
the number of addresses is potentially unbounded,
and establishing global invariants like the preservation of the sum of the balances by operations like transfer requires higher order reasoning.
In particular, automated reasoners do not provide ways to explicitly
specify summations as summation goes outside first-order logic and
drastically complicates reasoning. 


%Innovation
In this paper, we present a generalization of first-order logic which allows us to express 
the unbounded sum of balances. We prove the decidablity of one of our extensions and the
undecidability of a slightly richer one.  
We introduce first-order encodings which enable automated
reasoning over software transactions with summations.
%enables applying existing SMT solvers to reason about summations.
We demonstrate the applicability of our results by using SMT solvers
and first-order provers for validating the correctness of common transitions appearing in smart contracts.


==> includes/references.tex <==





% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)

%\bibliographystyle{IEEEtran}
\bibliography{includes/references}


==> includes/title.tex <==
Temporary Title of Paper to be Replaced at a Later Date, it is Deliberately Long in order to See How it Looks
